Evaluating Generalizability of Fine-Tuned Models for Fake News Detection

The Covid-19 pandemic has caused a dramatic and parallel rise in dangerous misinformation, denoted an `infodemic' by the CDC and WHO. Misinformation tied to the Covid-19 infodemic changes continuously; this can lead to performance degradation of fine-tuned models due to concept drift. Degredation can be mitigated if models generalize well-enough to capture some cyclical aspects of drifted data. In this paper, we explore generalizability of pre-trained and fine-tuned fake news detectors across 9 fake news datasets. We show that existing models often overfit on their training dataset and have poor performance on unseen data. However, on some subsets of unseen data that overlap with training data, models have higher accuracy. Based on this observation, we also present KMeans-Proxy, a fast and effective method based on K-Means clustering for quickly identifying these overlapping subsets of unseen data. KMeans-Proxy improves generalizability on unseen fake news datasets by 0.1-0.2 f1-points across datasets. We present both our generalizability experiments as well as KMeans-Proxy to further research in tackling the fake news problem.

==> Makefile <==
# Makefile for LaTeX files

PACKAGE=acmart

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
PANDOC = pandoc

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

PDFPICS :=
#PDFPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.pdf$$/) { print "$$foo[2] "; } else { print "$$foo[2].pdf "; }}' *.tex)
DEP	= *.tex

TRG	= $(SRC:%.tex=%.pdf)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

all 	: $(TRG)

define run-latex
	  $(COPY);$(LATEX) $<
	  egrep -q $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	  $(RM) $(<:%.tex=%.toc.bak)
	  # Display relevant warnings
	  egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

$(TRG)	: %.pdf : %.tex $(DEP) $(PDFPICS) $(BIBFILE)
	  @$(run-latex)

.PHONY	: all show clean ps pdf showps text stylecheck spellcheck

view:
	acroread $(PDF)

osx:
	open $(PDF)

text: *.tex
	$(PANDOC) --wrap=none -s $< -o $@

doc: *.tex
	$(PANDOC) --wrap=none -s $< -o $@

combined:
	pdfunite response.pdf logging.pdf combined.pdf

# Check style:
stylecheck:
	printf "weasel words: "
	sh ./scripts/weasel *.tex
	printf "\npassive voice: "
	sh ./scripts/passive *.tex
	printf "\nduplicates: "
	perl ./scripts/dups *.tex
	printf "\ndone\n"

# Check spelling with aspell
spellcheck:
	find . -name "*.tex" -exec aspell --lang=en --mode=tex --dont-suggest --personal=./.aspell.en.pws check "{}" \;

######################################################################
# Define rules for PDF source files.
%.pdf: %.eps
	epstopdf $< > $(<:%.eps=%.pdf)


docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.bak

distclean: docclean
	$(RM)  *.pdf 

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.pdf=%.aux) $(TRG:%.pdf=%.bbl) $(TRG:%.pdf=%.blg) $(TRG:%.pdf=%.log) $(TRG:%.pdf=%.out)

bclean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.pdf=%.aux) $(TRG:%.pdf=%.blg) $(TRG:%.pdf=%.log) $(TRG:%.pdf=%.out)


zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*' -x 'figs/*'
